Block mapping class groups and their finiteness properties

A Cantor surface $\mathcal C_d$ is a non-compact surface obtained by gluing copies of a fixed compact surface $Y^d$ (a block), with $d+1$ boundary components, in a tree-like fashion. For a fixed subgroup $H<Map(Y^d)$ , we consider the subgroup $\mathfrak B_d(H)<Map(\mathcal C_d)$ whose elements eventually send blocks to blocks and act like an element of $H$; we refer to $\mathfrak B_d(H)$ as the block mapping class group with local action prescribed by $H$. The family of groups so obtained contains the asymptotic mapping class groups of \cite{SW21a,ABF+21, FK04}. Moreover, there is a natural surjection onto the family symmetric Thompson groups of Farley--Hughes \cite{FH15}; in particular, they provide a positive answer to \cite[Question 5.37]{AV20}. We prove that, when the block is a (holed) sphere or a (holed) torus, $\mathfrak B_d(H)$ is of type $F_n$ if and only if $H$ is of type $F_n$. As a consequence, for every $n$, $Map(C_d)$ has a subgroup of type $F_n$ but not $F_{n+1}$ which contains the mapping class group of every compact subsurface of $\mathcal C_d$.

==> tikfig.tex <==
%\begin{figure}[h]\label{fig:ele-V}
%\centering
%\begin{tikzpicture}[line width=1pt, scale=0.4]
%\begin{scope}[xshift= -4cm]
 % \draw
  % (-12,-2) -- (-9,0) -- (-6,-2)
   %(-9,0) -- (-9,-2)
   %(-11,-1.33) -- (-11,-2)
   %(-11,-1.33) -- (-10,-2)
%   (-4,-2) -- (-1,0) -- (2,-2)
 %  (-1,0)  -- (-1,-2);
%
%\draw[dotted] (3.5,0)  -- (3.5,-3);

%  \filldraw
%  (-12,-2) circle (1.5pt)
%  (-9,0) circle (1.5pt)
%   (-6,-2) circle (1.5pt)
%   (-9,-2) circle (1.5pt)
%  (-11,-1.33)  circle (1.5pt)
%   (-11,-2) circle (1.5pt)
%   (-10,-2) circle (1.5pt)
%    (-4,-2) circle (1.5pt)
%   (-1,0) circle (1.5pt)
 %  (-1,-2) circle (1.5pt)
  % (-3.5,0) circle (1.5pt)
%   (2,-2) circle (1.5pt);
%  \node at  (-12,-2.5) {$1$};
%  \node at (-11,-2.5) {$2$};
%  \node at (-10,-2.5) {$3$};
%  \node at (-9,-2.5) {$4$};
%  \node at (-6,-2.5) {$5$};
%  \node at (-4,-2.5) {$6$};
%  \node at (-1,-2.5) {$7$};
%  \node at (2,-2.5) {$8$};
%\end{scope}

 % \begin{scope}[ xshift=13cm]
 %  \draw
  % (-12,-2) -- (-9,0) -- (-6,-2)
 %  (-9,0) -- (-9,-2)
   
 % (-8,-2) -- (-9,-1.33) -- (-10,-2)
   
%   (-4,-2) -- (-1,0) -- (2,-2)
%   (-1,0)  -- (-1,-2);

 % \filldraw
%  (-12,-2) circle (1.5pt)
%  (-9,0) circle (1.5pt)
%   (-6,-2) circle (1.5pt)
%   (-9,-2) circle (1.5pt)
%  (-9,-1.33)  circle (1.5pt)
%   (-10,-2) circle (1.5pt)
%   (-8,-2) circle (1.5pt)
%    (-4,-2) circle (1.5pt)
%   (-1,0) circle (1.5pt)
%   (2,-2) circle (1.5pt)
%   (-1,-2) circle (1.5pt);
%  \node at  (-12,-2.5) {$4$};
 % \node at (-6,-2.5) {$6$};
%  \node at (-10,-2.5) {$1$};
%  \node at (-8,-2.5) {$3$};
%  \node at (-9,-2.5) {$2$};
%  \node at (-4,-2.5) {$7$};
%  \node at (2,-2.5) {$8$};
%  \node at (-1,-2.5) {$5$};
% \end{scope}

%  \begin{scope}[ yshift=-4.5cm,xshift= -4cm]
%    \draw
%   (-12,-2) -- (-9,0) -- (-6,-2)
%   (-9,0) -- (-9,-2)
  % (-11,-1.33) -- (-11,-2)
  % (-11,-1.33) -- (-10,-2)
%   (-4,-2) -- (-1,0) -- (2,-2)
%   (-1,0)  -- (-1,-2);

%\draw[dotted] (3.5,0)  -- (3.5,-3);

%  \filldraw
%  (-12,-2) circle (1.5pt)
%  (-9,0) circle (1.5pt)
%   (-6,-2) circle (1.5pt)
%   (-9,-2) circle (1.5pt)
  %(-11,-1.33)  circle (1.5pt)
  % (-11,-2) circle (1.5pt)
  % (-10,-2) circle (1.5pt)
%    (-4,-2) circle (1.5pt)
%   (-1,0) circle (1.5pt)
%   (-1,-2) circle (1.5pt)
  % (-3.5,0) circle (1.5pt)
%   (2,-2) circle (1.5pt);
%  \node at  (-12,-2.5) {$1$};
 % \node at (-11,-2.5) {$2$};
 % \node at (-10,-2.5) {$3$};
%  \node at (-9,-2.5) {$2$};
%  \node at (-6,-2.5) {$3$};
 % \node at (-4,-2.5) {$4$};
%  \node at (-1,-2.5) {$5$};
%  \node at (2,-2.5) {$6$};
%  \end{scope}

%  \begin{scope}[xshift=13cm, yshift=-4.5cm]
%   \draw
%   (-12,-2) -- (-9,0) -- (-6,-2)
%   (-9,0) -- (-9,-2)
   
  %(-8,-2) -- (-9,-1.33) -- (-10,-2)
   
%   (-4,-2) -- (-1,0) -- (2,-2)
%   (-1,0)  -- (-1,-2);
%
%  \filldraw
%  (-12,-2) circle (1.5pt)
%  (-9,0) circle (1.5pt)
%   (-6,-2) circle (1.5pt)
%   (-9,-2) circle (1.5pt)
 % (-9,-1.33)  circle (1.5pt)
  % (-10,-2) circle (1.5pt)
  % (-8,-2) circle (1.5pt)
%    (-4,-2) circle (1.5pt)
%   (-1,0) circle (1.5pt)
%   (2,-2) circle (1.5pt)
%   (-1,-2) circle (1.5pt);
%  \node at  (-12,-2.5) {$2$};
%  \node at (-6,-2.5) {$4$};
 % \node at (-10,-2.5) {$1$};
%  \node at (-8,-2.5) {$3$};
%  \node at (-9,-2.5) {$1$};
%  \node at (-4,-2.5) {$5$};
%  \node at (2,-2.5) {$6$};
%  \node at (-1,-2.5) {$3$};
%  \end{scope}
%\end{tikzpicture}


%\caption{Reduction, of the top paired $(3,2)$-forest diagram to the bottom one.}
%\label{fig:reduction_V}
%\end{figure}
